Same Stats, Different Graphs (Graph Statistics and Why We Need Graph Drawings)

Data analysts commonly utilize statistics to summarize large datasets. While it is often sufficient to explore only the summary statistics of a dataset (e.g., min/mean/max), Anscombe's Quartet demonstrates how such statistics can be misleading. Graph mining has a similar problem in that graph statistics (e.g., density, connectivity, clustering coefficient) may not capture all of the critical properties of a given graph. To study the relationships between different graph properties and statistics, we examine all low-order (<= 10) non-isomorphic graphs and provide a simple visual analytics system to explore correlations across multiple graph properties. However, for graphs with more than ten nodes, generating the entire space of graphs becomes quickly intractable. We use different random graph generation methods to further look into the distribution of graph statistics for higher order graphs and investigate the impact of various sampling methodologies. We also describe a method for generating many graphs that are identical over a number of graph properties and statistics yet are clearly different and identifiably distinct.

==> images/conclusion.tex <==
\section{Conclusions and Future Work}



==> images/correlations.tex <==
\section{An Analysis of Graph Statistics}
Plots of the statistics and correlations for the graphs. Discussion of trends as number of nodes increases. Finish section with $|V| = 10$ example and how many graphs have the exact same statistics, and show what they look like.

Figure \ref{fig:full_convex_hull} shows a distribution of the values of all pairs of graph properties for number of nodes $N \in \{5, 6, 7, 8, 9, 10\}$. Each cell of the matrix shows the convex hull of distribution of these values. For majority of the cells, we find that the distribution or the coverage of values expands with increasing $N$. Figure \ref{fig:coverage_comparison} shows this patterns for three pairs of properties. This increase in coverage informs the fact that it is possible to get a higher range of one property value while we fix another property value from the pair if the number of nodes increase. 

Figure \ref{fig:correlation_vs_n} shows how correlation values between all pairs of properties change when the number of nodes($N$) in the graph are increased from $N = 5$ to $N = 10$. The trend line for the ground truth data shows correlation values calculated using the set of all possible graphs for a given number of nodes. Separate trend lines are also presented for correlation values calculated from graphs generated through the Erdos-Renyi (ER) model. For these graphs generated by the ER model, each line corresponds to the graphs with the count either $1\%$, $5\%$ or $10\%$ of the total number of graphs for each $N$(or simply $10$ graphs if the percentage yields less than $10$ graphs). 

For each cell of the matrix, the value of correlations converge towards the similar value after $N=8$, for the ground truth and ER-model generated graphs. The correlation values for the ground truth data show a variety of trends. For example, correlation values are almost for the pair average clustering coefficient and square clustering coefficient. In contrast, the correlation values increase with an increase in $N$ for assortativity and average path length. Most cells however, show a decrease in correlation with increasing $N$.

\begin{figure} [tbh]
\includegraphics[width=\linewidth]{./images/full_convex_hull.png}
\caption{Convex hull of the distribution of values for all pairs of graph properties}
  \label{fig:full_convex_hull}
\end{figure}

\begin{figure} [tbh]
\centering
\includegraphics[width=0.75\linewidth]{./images/coverage_comparison.png}
\caption{Expansion of coverage of properties with increasing $N$(top to bottom)}
  \label{fig:coverage_comparison}
\end{figure}

\begin{figure} [tbh]
\includegraphics[width=\linewidth]{./images/corr_gt_ER.png}
\caption{Trends in correlation of graph properties with increasing $N$. The X-axis provides the number of nodes, while the Y-axis gives the correlation value for the pair of graph properties}
  \label{fig:correlation_vs_n}
\end{figure}

==> images/fixPropStillDiff.tex <==
\section{Generating Different Graphs with several Identical Statistics}

For finding the different graphs with several same statistics, we directly use the all small non-isomorphic graphs. However, this approach gets stuck when $|V|\geq 10$, since non-isomorphic graph set for $|V|\geq 10$ are huge. The replace approach is that generate graphs by graph generators and using filter to find different graphs with several same statistics.

\subsection{Generating Graphs by all non-isomorphic graphs}

For $|V|\leq 10$, we directly use all possible non-isomorphic graphs as our data set. By using this data set, we are able to fix more than 5 statistics and properties, but still get several distinct statistics. For convenient, we generate a plot which separates the variability of statistic in 10 slots. in each slot, there is one graph drawing by spring layout[TODO: SHOULD WE CITE A REFERENCE FOR SPRING LAYOUT?]. it represent the graph with a specific statistics. 

For the first experiment, we fix $|v| = 9$ $APL\in$ (1.425,1.475), $density\in$ (0.525,0.575), $GCC\in$ (0.5,0.6), $r_t\in$ (0.15,0.25). We also let the graph not regular, tree, bipartite and Eulerian. We know assortativity should be a value between -1 to 1. In this case, each slot  has a range of 0.2. Therefore, we can represent the whole range of assortativity by using 10 slots.

\begin{figure}
\includegraphics[width=\linewidth]{./images/fix_5_ass.PNG}
\caption{assortativity variability.[TODO: HANG WILL UPDATE NEW PLOTS WHICH INCLUDE ASS VALUE]}
\end{figure}

From figure 9, we are able to collect a graph set, which almost covers all the varying of assortativity.  From looking those slots, it is oblivious that the most left graph is different from the most right graph. either from assortativity or spring layout visualization. Hence, based on ground-truth graph set with $|V|$ = 9, we are able to fix 5 boolean value statistics and 5 statistics on the matrix, and able to varying assortativity from -0.75 to 0.6. Therefore, we can conclude that there are graph sets satisfy our requirement not only when $|V|$ be big, but for small $|V|$. 

Similarly figure \ref{}, shows graphs with varying global clustering coefficient value from 0.18 to 0.65. However the graphs are very similar on other statistics: average path length(1.52 to 1.54), diameter(3), node connectivity(2), edge connectivity(2), assortativity(-0.21), density(0.50 to 0.52). 

% For second experiment
% \begin{figure}
% \includegraphics[width=\linewidth]{./images/fix_5_gcc.PNG}
% \caption{GCC variability.[TODO: HANG WILL UPDATE NEW PLOTS WHICH INCLUDE GCC VALUE]}
% \end{figure}
 

\subsection{Generating Graphs by Graph Generators}
The replace approach is using generators to build the data set and using filter to find different graphs with several same statistics. 

\subsubsection{Graph Generator with Desired Property Distribution} $\newline$
For two most important property of graph, $|V|$ and $|E|$, we generate all graphs with same $|V|$ and properly choose $|E|$ by consider the following two methods.
\begin{enumerate}
\item select $|E|$ uniformly from it range. this is equivalence to force graph density in the generating set follows uniformly distribution, named it uniform method
\item select $|E|$ by force it to a distribution which similar to its ground truth graph set, name it population method
\end{enumerate}
For Erd\"os-R\'enyi, we draw TODO: WHAT SHOULD I WRITE HERE?
\begin{figure}
\includegraphics[width=\linewidth]{./images/sdd.png}
\caption{Statistics Density Distribution}
\end{figure}

From the plot above, the graphs generated by population method 

For Watts and Strogatz (WS) model and Barabasi and Albert (BA) model, we cannot force the edge to the whole range, also unable to force the distribution either Uniform or follows ground truth edge distribution. the graphs generated by WS model can only have $|E|$ = $k*|V|$. So for $|V|$ = 9, the edge can only be 9, 18, 27 and 36. Similar thing for BA model, the graphs generated by BA has $|E|=k*(|V|-k)$. For $|V|$=9, the edge can only be 8,14,18 and 20. There is no reason that those two generators are able to cover most of variability of statistics. 


\subsubsection{Generators Performance at Ground Truth $|V|$ = 9} $\newline$
We examine all three generators and decide to use Erd\"os-R\'enyi with selecting edge number uniformly. 

==> images/graphgenerators.tex <==
\section{Graph Statistics and Graph Generators}
In here, we select four different random generators, which are Erdo\"s-Rényi model, Watts–Strogatz small-world model, Barabási–Albert preferential attachment model, which cover most type of generator models. Optimization-Based Models, which is the one we did not cover, provide a very intuitive process that leads to both power laws and resilience. intuitively, this model would give more specific graphs based on Preferential Attachment Models, which only guarantee power-law. We believe Barabási–Albert is able to represent the variability of Optimization-Based Models. 

 We employ a general strategy: start fixing one statistic and check what another statistic can vary. If the generators give broad distribution ranges for other statistics when we fix one statistic. We can continue doing that and find the graphs set we need. The first statistic we considered is density. We fix $|v|=50$ and vary the edge in order to see the range of other statistics based on the different percentage of density. We first do 1 percentage increment. For each percent of density, we generate 100,000 graphs for each random graph generators. The first statistic we check is GCC. We believe there do not have a strong correlation. Intuitively,  There exists a huge amount possibility, which allows GCC = 0 and GCC is a big number for a fixed density.especially for density in 30-60\%. However, the expected result does not appear. For all random generators, we are failed to give a distribution that we fixed density and the GCC can still vary from 0 to 1. However, from real life graph set, we know the relationship between GCC and density is not strong. Which contradict to the result from the generator

This above result implies that all generators may provide bias sample from ground-truth graph set. Before we fix the special statistics to see what other statistics tend to different, we should figure out the relations between each statistic. Some statistics are highly correlated with another, without knowing their relation, we need to guess what the relation is. This will make us hard to distinguish whether the generators give bias sample or the distributions for those two statistics themselves has a strong correlation. We guessed the density and GCC does not have a strong correlation. The generator’s experiment implies that there exists a strong correlation between GCC and density. In order to escape from this situation, we should know what statistics are able to change when others are fixed. From Garcia et al.~/cite{garcia2013correlation} works, correlation analysis for summary statistics gives a further information for choosing statistics and the value of statistics. Therefore, it is worth to study a graph set, which covers all probabilities of one specific $|v|$. We call it ground-truth graph set


Comparing with ground-truth graph set, Using generators to create a graph set is easy and quick, however for the ground-truth graph set we can only create and test our property in a small $|v|$; once the $|v|$ is big it is impossible to get and process a graph set. So, the generator performance for converging ground-truth graph set is important. In the last section, we talked about the random generators and ground-truth graph set. Now, we are ready for testing the ability of representation.  

In order to figure out how good of each random generator does, we decide to continue using the ground-truth graph set with $|v|$ = 9(the one we used in the last section, consider this graph set as the aim for coverage). For each random generator, we try to make the generator as random as possible and check the range of each statistic. Be aware, all four generators implementations come from networkX. ~\cite{hagberg2008exploring}

 

For Erdős-Rényi graph, it require 2 parameters,"{\em n}" number of vertex and "{\em p}" probability for edge creation in range. So we pick {\em "n" }= 9 and random pick a value from 0 to 1 for {\em "p" }.

For Watts–Strogatz small-world graph, it require 3 parameters, ,{\em "n"}: number of vertex {\em "k"}:  Each node is joined with its {\em k} nearest neighbors in a ring topology  and {\em "p"}: probability for edge creation in range. So we pick {\em "n" = 9}, pick k from 2 to $|v|-1$ and random pick a value from 0 to 1 for "{\em p}".

For the Barabási–Albert preferential attachment model, it requires 2 parameters,"{\em n}" number of vertexes and "{\em m}" edges to attach from a new node to existing nodes. So we pick {\em "n" = 9} and random pick a integer value from 1 to n-1 for {\em "m" }. Noted, the whole range of m is from 1 to n-1.

For geometric graph, it requires 2 parameters,"{\em n}" number of vertex and "{\em radius}" Distance threshold value. So we pick {\em "n" = 9} and random pick a value from 0 to 1 for {\em "radius" }.


\subsection{Coverage for Ground-Truth Graph Set}

For each generator, we test 1\%, 0.1\% and 0.01\% number of ground-truth graph set. Because graph set with a large $|v|$ is impossible to generate 10\% or even 1\% of graphs. In section 5.2, we discussed how quick of non-isomorphic graphs goes for number of vertex. it is reasonable to only give a little percentage of graph compare to its ground-truth graph set even $|v|$ is small. In the following section, we test their coverage at different levels by two ways.

Intuitively, we can measure the coverage of random generators by drawing ground-truth graph set in the first, then draw generator graph set after and see how well the generator set cover ground-truth graph set. We further give blue color for ground-truth graph set and red to the generator set. Because, the graph-truth graph set includes all possible of graphs for a fixed $|v|$. There is at least 1 bluepoint under each redpoint. we did several comparisons in the appendix.  



More Than just looking at the coverage, test the increasing of $|$V$|$ under Erdős-Rényi graph is also important. there are many way to select the random method, 2 most important random method are Uniform pick $P$ and let the graph follow exactly same distribution as it's population edge distribution.

Uniform distribution is easy to apply. it only ask $p$ being uniform distribution. following population edge distribution is not easy as uniform. We need to use population edge distribution as weight and then using the weight random.
\begin{figure}
\includegraphics[width=\linewidth]{./images/ER_Uniform_7-10.png}
\caption{ER follow with uniform.}
\end{figure}
\begin{figure}
\includegraphics[width=\linewidth]{./images/ER_Population_7-10.png}
\caption{ER follow with ground truth edge distribution}
\end{figure}

From the Uniform matrix(figure 8), most correlations coverage have almost  same space as ground-truth. Different from Uniform, the one following ground truth edge distribution(figure 9) does not do a good job. Pearson correlation(the number on the right of each plot) for most plots does not follow the same tread as ground truth one. 


% From appendies  

Another way to measure how good the generator represents the graph is using Kullback–Leibler divergence or distance test like Kolmogorov-Smirnov test.


==> images/introduction.tex <==
\section{Introduction}
\begin{wrapfigure}{r}{0.4\textwidth} \vspace{-1.4cm}\includegraphics[width=.4\textwidth]{./images/Anscombe_s_Quartet.png}
\caption{Anscombe's Quartet. All four graphs share the same mean and standard deviation in x and y.}
\centering
\end{wrapfigure}Statistics are often used to summarize a large dataset. In a way, one hopes to find the ``most important" statistics that capture one's data. For example, when comparing two countries, we often specify the population size, GDP, employment rate, etc. The idea is that if two countries have a ``similar" statistical profile, they are similar. For example, France and Germany may have a more similar demographic profile than the United States and France. However, Anscombe's quartet~\cite{Anscombe}, Figure 1, countered the impression among statisticians about the exactness of numerical calculations and expressed the value of using graphical representations when describing datasets. More recently, work by Matejka and Fitzmaurice~\cite{matejka2017same} further demonstrated the need for visualizing data by creating a dataset generation method that can mutate a dataset while keeping its summary statistics but greatly change its visual form on scatterplots.

%\begin{figure} [tbh]
%\includegraphics[width=\linewidth]{./images/1}
%\caption{In these four graphs we have the same number of vertices $|V| = 12$, the same number of edges $|E| = 21$, the same number of triangles $\bigtriangleup=10$, and all the graphs are connected, non-Eulerian, non-bipartite, with average path length APL $ \in (2.43,2.53)$, and global clustering coefficient GCC $ \in (0.48, 0.53)$. However, structurally the graphs are very different. For example, two of the graphs are planar and the other two are not, some show regular patterns and are symmetric, others are not and their degree assortativity is very different.}
%  \label{similar stat 1}
%\end{figure}

%\begin{figure}[t]
\begin{wrapfigure}{r}{0.61\textwidth} \vspace{-.9cm}
\fbox{\includegraphics[width=0.28\textwidth]{./images/8.PNG}}\fbox{\includegraphics[width=0.28\textwidth]{./images/11.PNG}}
\fbox{\includegraphics[width=0.28\textwidth]{./images/3.PNG}}%\hspace{1.9cm}
\fbox{\includegraphics[width=0.28\textwidth]{./images/12.PNG}}
  \caption{These four graphs share the same 5 common statistics: number of vertices $|V| = 12$, number of edges $|E| = 21$, number of triangles $|\bigtriangleup|=10$, girth $=3$ and global clustering coefficient {\em GCC}$=0.5$.
  %further, all the graphs are non-Eulerian and non-bipartite. %with average path length APL $ \in (2.43,2.53)$, and global clustering coefficient GCC $ \in (0.48, 0.53)$.
 However, structurally the graphs are very different: three of the graphs are planar and the fourth one is not, some show regular patterns and are symmetric, others are not. Finally, one of the graphs is disconnected, another is 1-connected and the rest are 2-connected.}
 %and their degree assortativity is very different.}
\label{similar stat 1}
\end{wrapfigure}

Similarly, in the graph analytics community, a variety of statistics are being used to summarize graphs, such as average path length, global clustering coefficient, etc. However, graph statistics suffer the same issues posed by Anscombe. In Figure 2, we provide an illustration of the same stats, different graphs problem. Here, we show four graphs, each with the same number of vertices and edges. One graph is un-connected, another non-planar, another symmetric. Clearly, these graphs are dramatically different, yet they all share common statistical properties (same number of triangles, similar average path link, similar global clustering coefficient). As such, exploring the graphical representations is as critical for graph analysis as for traditional statistical analysis.

%Recently, Matejka and Fitzmaurice~\cite{matejka2017same} proposed a dataset generation method that can mutate a dataset while keeping its summary statistics but greatly change its visual graphs on scatterplots. These works demonstrate the value of visualization and graph drawing in that a proper visual display would be able to compensate the deficiency of statistic descriptions. %Graph Drawings could visually reveal some properties of the underlaying data and show the structure of graphs (or network data). Therefore, in nature, we would like to see if graph drawings can be used to assist the interpretation of graph statistic properties, such as clustering coefficient.  

This begs the question of whether a graph generation approach in the vein of Matejka and Fitzmaurice~\cite{matejka2017same} can also be developed. From our examples of Figure 2, it is clear that for at least some graph properties, there exist drastically different types of graphs that share similar statistics. With this in mind, we first consider how can we fix a few graph statistics (such as number of nodes, number of edges, number of triangles) and vary another statistic (such as, clustering coefficient). We find that there is a spectrum of possibilities: sometimes the ``unrestricted" statistic can vary dramatically, sometimes not, and the outcome depends on two issues: (a) the inherent correlation between some statistics (e.g., density and number of triangles), and; (b) the bias in graph generators.

Due to the inherent correlation between some graph statistics, we study the correlation between graph summary statistics across the set of all graphs that can be generated from $|V| = 5$ to $|V|=10$ ($|v|$: number of vertices). The statistical properties derived for all graphs for a given number of nodes provide further information about ``restrictions". In other words, the range of one statistic may be restricted if another statistical property is fixed. However, we cannot explore the entire space of graph statistics and correlations. As the number of nodes grows, the number of different non-isomorphic graphs grows super-exponentially. For $|V|=1, 2 \dots 9$ the numbers are $1, 2, 4, 11, 34, 156, 1044, 12346, 274668$, but for $|V|=16$ we have $64001015704527557894928$ non-isomoprhic graphs.
%|V|=24 we have $195704906302078447922174862416726256004122075267063365754368$.  

As such, the bias in generating graphs at random is critical. We study how well sampling using random generators will represent the whole graph set for an arbitrary number of nodes with respect to their coverage of the graph statistics. One way to evaluate the performance of random generators is based on the ground-truth graph set (e.g., the set of all non-isomorphic graphs that can exist for $N$ nodes). Using ground-truth graph sets from $|V|=5$ to $|V|=10$, we have all possible graphs for a specific $|v|$. If we randomly generate a small set of graphs using a given graph generator, we can explore how well the sample and generator cover the space of graph statistics. In this way, we can begin exploring the issues of ``same stats, different graphs'' for all numbers of nodes.

%We can plot the graphs from generators with fixed $|v|$ and ground-truth graph set with same $|v|$. Then, comparing their different by looking at the matrix. Further, we study Those random generators based on the matrix by increasing the $|v|$. As I will explain in Section 5.2, it is impossible to draw ground-truth graph set due to too many possibilities. For big $|v|$, random generators cannot represent the graph set properly. From one ground-truth graph set, we are able to construct a subset for which all graphs inside have 5 restricted statistics, and one extremely different.
    
%However, the range limitations of certain graph statistics when keeping others constant is not completely clear. In this paper, we use the complete ground-truth datasets (i.e., the set of all possible non-isomporphic graphs that could exist for a given number of vertices) for $|V|=5$ to $|V=10|$ to explore the relationships between various graph statistics (some are obvious, and others are not). We then explore how  ... NEED TO BE CLEAR ON WHY WE WANT TO DO THE SAMPLING STUFF ... STEPHEN, CAN YOU HELP HERE?

%Unfortunately, common graph drawing algorithms may not always be able to adequately show the differences in statistics between two graphs. While graph drawing algorithms have focused on minimizing edge crossing or depicting symmetry, little work has explored how well a user can discriminate various graph prperties. Soni et al.~\cite{soni2018perception} studied the perception ability of graph density and local clustering coefficient when the data is visualized using different graph drawing algorithms. Results from this study indicated that some graph drawing algorithms may be more appropriate than others when trying to help users perceive differences between underlying graph statistics. However, could be more appropriate than others to better perceive the difference in clustering coefficient, we also noticed that some graph statistics are correlated in the dataset and some could very a lot.  Therefore, to better understand the need of graph drawing in terms of graph property analysis, we need to first answer some questions. Among these widely used graph statistical properties, are there any correlations between them so that the change of one could greatly impact the change of another? When some properties are controlled, to what extend some other properties can vary, and how would this affect the visual display of graph drawing? In this paper, we use experimental method to study the correlation of a list of graph properties and more importantly we will explore the cases that when some graph statistics are fixed some other statistics could still vary a lot and the graphs could end up being drew differently. 


%Possible questions to ask: are graph generators cover the desired property value range and distribution? How many properties should we consider in order to define a graph (in the visual display)?




==> images/preliminary.tex <==
\section{Preliminary Experiments and Findings}
%We can use EuroVis paper graph set to start this motivation. Given those generators, our graphs have obvious correlated statistical properties. This motivated us to look at the graph property correlation and the distribution of given generators.
%As previously stated, one of our goals is to be able to generate 

In our recent work on graph property and graph layouts, we limited ourselves to graph order = 100 and controlled graph density and the average local clustering coefficient in two experiments~\cite{soni2018perception}. Analyzing these published datasets (http://vader.lab.asu.edu/GraphAnalytics/), we found some interesting patterns among the statistics described in Table~\ref{Table:properties}. 

\begin{figure}[t]
\centering
\includegraphics[width = 0.49\textwidth]{images/corr2}
\hfill
\includegraphics[width = 0.49\textwidth]{images/corr1}
\caption{Graph property correlation matrix plots for the edge density dataset (left) and the average clustering coefficient dataset (right). }
\label{Fig:heatmap}
\end{figure}

The edge density dataset has 4,950 graphs and the average clustering coefficient dataset has 3,450 number of graphs. The 10 properties are calculated for all these graphs, and their Pearson correlation coefficients are visualized in Fig~\ref{Fig:heatmap}. We observed high correlations either positive (green) or negative (red) in many property pairs. For example, average clustering coefficient is highly correlated to all other properties in the edge density dataset except assortativity, and it is also highly correlated to global clustering coefficient and the number of triangles in the average clustering coefficient dataset. 

However, these graphs were developed for a very specific purpose, and cover only an extremely limited space of all graphs with $|V|=100$. Two factors likely impact these correlations: the generator used, and the statistical properties that were controlled (e.g., insuring the number of edges remained constant). For the edge density graph set, we used a random graph generation algorithm that varies the number of edges while keeping a uniform probability of connecting two nodes.  For the average clustering coefficient graph set, we controlled graph density and degree distribution (power-law). This motivated us to conduct the following explorations.
\begin{enumerate}
\item Generate all isomorphic lower order graphs ($|V|\leq 10$) and analyze the relationships between statistical properties. This shall be considered as ground truth due to its completeness.
\item Use popular graph generators to create a sample of graphs and compare the graph property distributions of these outputs to the ground truth. This depicts the characteristics of different graph generators in terms of graph property coverage and helps us to think about which generator should we use in different scenarios.
\end{enumerate}

==> images/relatedwork.tex <==
\section{Related Work}
Currently, a large number of graph statistics and graph generation methods have been developed. As graphs become larger, our ability to adequately visualize graph properties becomes challenging. As such, it is critical to understand the relationships between graph statistics, as well as the ability of a graph generator to cover the range of statistical properties for a given sample size.

%Dataset is depicted by exact statistical measures, and in the meanwhile, visualization provides an intuitive approach to look at the data. Studies have shown that although statistics of two datasets are same, their visual representation could be different greatly~\cite{Anscombe,matejka2017same}. The classical example is the four datasets create by Anscombe~\cite{Anscombe} where they share the same XXX but looks dramatically different in scatterplots.  Matejka and Fitzmaurice~\cite{matejka2017same} further proposed a systematic approach to generate such datasets where a certain statistics are fixed but their 2D scatterplots have totally different visual patterns. From these examples we see that graphs can be used together with statistical analysis to illustrate the underlying dataset. Following this, there are two ways of exploring the effectiveness of graph drawing. First, researchers were trying to understand which graph drawing method best line up with the perception of a given statistical property, and second, we also see the need of using visualization to depict the facet of the dataset which cannot be shown by summary statistics. 
%[I PROPABLY SHOULD START WITH THIS TWO ASPECTS.]

%Correlation perception study

%Our Eurovis study

%[GRAPH LAYOUTS AND THEIR STRENGTH.] \textcolor{red}{Personal notes: Here I can first start with how layouts try to conform to an aesthetic or reduce computational cost, but then also talk about certain graph layout that are great for perceiving certain properties like cc with FD-layout.}
\input{input/propertytable}

\subsection{Graph Statistics}
%This subsection discusses important graph statistics, their applications, and some (if any) studies on their correlations.  We will also talk about our EuroVis paper to link the graph statistics analysis to graph drawings. 
%Existing studies on how different visual displays are for the same stats datasets mainly focused on 1D and 2D statistics with scatterplots, while little attention has been put on analyzing graph statistics and graph drawings. In the work by Soni et al.~\cite{soni2018perception}, we see that different graph drawing approaches have different ability of visually expressing graph statistics, and their experiments inspired us to look at the statistics of graph (node-link) datasets and how differently graph drawings are when the data shares the same graph statistics.
%[TRY TO GROUP PROPERTIES AS : 1. GENERAL PROPERTIES, DENSITY, TRIANGLES 2. PROPERTIES FOR CERTAIN TYPE OF NETWORK, CC, AVERAGE PATH LENGTH - ALSO ADD IN THE NICE TABLE THAT HANG HAD]
%and then to explore certain types of networks, there are graph generators to sacrifice some properties.  Introduce the different generators here. 

Graphs, in general, can be very complex to directly understand and explore. However, certain statistical measures have been developed that give useful insights on the structural properties of a graph. Some of these properties, along with their definition, has been compiled in Table~\ref{Table:properties}. These properties range from basic ones, such as vertex count, edge count, and graph density, to complex ones, such as clustering coefficients and average path length.

%There are some basic graph properties that characterize the topology of the network like vertex count, edge count, triangle count, average degree, graph density, vertex connectivity, edge connectivity, diameter, radius, etc. %From the definitions in Table, clearly edge count, average degree and graph density are closely related. 
There are two properties that are necessary to describe any graph: the number of nodes and the number of edges. As such, the properties are often used to dervie other simple measures. For example, graph density is the ratio edges to nodes, and real-world networks are often found to have a low graph density~\cite{melancon2006just}. Node connectivity and edge connectivity measures may be used to describe the resilience of a network~\cite{cartwright1956structural,loguinov2003graph}, 
and graph diameter~\cite{hanneman2005introduction} describes the shortest distance by which every two points can be connected~\cite{albert1999internet,broder2000graph}. %Diameter measures the size of the network \cite{hanneman2005introduction} (i.e. number of steps required to move from one side of network to other). For example, \cite{albert1999internet,broder2000graph} studied the size of the huge World-Wide Web by estimating its diameter. 

Other graph statistcs measure how tightly nodes are grouped in a graph. For example, the clustering coefficient has been used to describe many real world networks, and can be measured locally and globally. Nodes in a highly connected clique tend to have a high local clustering coefficient, and a graph with clear clustering patterns will have a high global clustering coefficient~\cite{feld1981focused,frank1982cluster,karlberg1997testing,newman2003structure}.
%An alternative way to calculate the global clustering of a graph is to use the average clustering coefficient introduced by Watts and Strogatz \cite{watts1998collective}. 
Studies have shown that the global clustering coefficient (a.k.s. transitivity) has been found to be almost always larger in real-world graphs than in Erdos-Renyi graphs with same number of nodes and edges~\cite{chakrabarti2006graph,newman2003structure,uzzi2005collaboration}, and a small-world network should have a relatively large average clustering coefficient~\cite{davis2003small,ebel2002scale,watts1998collective}. 
Other than clustering coefficients, people also look at the average path length (APL) in the study of small-world networks where APL grows logarithmically with the graph order and most real-world networks exhibit a short average path length \cite{davis2003small,ebel2002scale,newman2003structure,uzzi2005collaboration,van2004yeast,watts1998collective}. 

Degree distribution is one frequently used property describing the graph degree statistics. Many real world networks, including communication, citation, biological and social networks, have been found to follow a power-law shaped degree distribution
%, i.e. $P(k) \sim Ak^{-\gamma}$ where $2 < \gamma < 3$ 
\cite{boccaletti2006complex,chakrabarti2006graph,newman2003structure}. Other real world networks have been found to follow an exponential degree distribution \cite{guimera2003self,sen2003small,wei2009worldwide}.
Assortativity is another property for graph degreee statistics.  It describes the preference of a node's connection to others and assortative coefficient is calculated as the Pearson correlation between node degrees of paired nodes~\cite{newman2002assortative}. A random graph generated by ER model will have a 0 assortative coefficient.   
Newman~\cite{newman2002assortative} extensively studied assortativity in real networks and found that social networks were often assortative (positive $A$), i.e. vertices with a similar degree preferetially connect together, whereas technological and biological networks tend to be disassortative(negative $A$) implying that vertices with a smaller degree tend to connect to high degree vertices. Moreover, assortativity has been shown to affect clustering \cite{maslov2004detection}, resilience \cite{newman2002assortative}, and epidemic-spreads~\cite{boguna2002epidemic} in networks.

 

\subsection{Graph Generators}
As was hinted in the graph statistics, these statistcs have been used to describe various classes of graphs (small-world, scale-free, etc.), and a variety of algorithms have been developed to automatically generate graphs that will mimic these various properties.
%The history of graph generators dates back to 1959 when Erd\"os and Renyi~\cite{erdos1959random} described the first model for random graphs based on adding any edge in the graph with a fixed probability $p\in [0,1]$. Surprisingly, this simple model allowed for the discovery of phenomena such as the phase transition of connectivity at $p=\log n/n$. This simple model fails to model ``real-world" networks that have different clustering structure and shorter average shortest paths. With this in mind, new models such as that of Watts-Strogatz and Barabasi-Albert were introduced. The Watts-Strogatz model, generates random graphs with small-world properties, and the Barabasi-Albert model, generates scale-free networks through preferential attachment.
Charkabati et al.~\cite{chakrabarti2007graph} divide graph models and generators into four broad categories:
\begin{enumerate}
\item Random Graph Models: The graphs are generated by a random process.
\item Preferential Attachment Models: In these models, the ``rich” get ``richer” as the network grows, leading to power law effects. 
\item Optimization-Based Models: Here, power laws are shown to evolve when risks are minimized using limited resources. 
\item Geographical Models: These models consider the effects of geography (i.e., the positions of the nodes) on the growth and topology of the network. This is relevant for modeling router or power grid networks, which involve laying wires between points on the globe. 
\end{enumerate}

The Erdo\"s-Rényi (ER) network model is a simple graph generation model\cite{chakrabarti2006graph} that generates graphs either by choosing a network randomly with equal probability from a set of all possible networks of size $N$ with $E$ edges\cite{gilbert1959random} or by creating each possible edge of a network with $N$ vertices with probability $P$ \cite{erdos1959random}. The latter process gives a binomial degree distribution and it can be approximated with Poisson distribution for large $n$. It is also possible to create networks where the degree follows other common probability distributions, such as the exponential distribution \cite{deng2011exponential} or Gaussian distribution \cite{javarone2015gaussian}. Moreover, networks with any given degree sequence can be generated using the configuration model \cite{newman2003structure}. 

Watts and Strogatz \cite{watts1998collective} developed the classical approach to generate small world graphs. This model could create disconnected graphs, but the variation suggested by Newman and Watts \cite{newman1999scaling} generates connected graphs. Subsequently, more models for generating small world networks were proposed including Faraz et al. \cite{zaidi2012generating}(the networks are additionally scale free), Jian-Guo et al. \cite{jian2006multistage}(the networks have a scaling exponent=$3$ and a very high clustering coefficient=$0.81$ for large $N$), and Faraz \cite{zaidi2013small}(clustering was introduced through cliques or densely connected vertices often found in real-world networks). 

Other various models have also been proposed for generating synthetic scale-free networks with a varying scaling exponent($\gamma$). The first scale-free network model was given by de Solla Price \cite{price1976general} which generated directed networks. Barabasi and Albert (BA)~\cite{barabasi1999emergence} is another popular network model for generating undirected networks. It is a network growth model in which each added vertex has a fixed number of edges $m$, and the probability of each edge connecting to an existing vertex $v$ is proportional to the degree of $v$. The scaling exponent of the BA model is $\approx -3$ \cite{dorogovtsev2000structure}. Dorogovtsev et al.~\cite{dorogovtsev2000structure} and Albert and Barabasi~\cite{albert2002statistical} also developed a variation of the BA model with a tunable scaling exponent. Dorogovtsev et al.~\cite{dorogovtsev2002accelerated} developed a scale-free network growth model where the number of edges of each new vertex increases with network's size.   

